On Dynamic Precision Scaling

Based on the observation that application phases exhibit varying degrees of sensitivity to noise (i.e., accuracy loss) in computation during execution, this paper explores how Dynamic Precision Scaling (DPS) can maximize power efficiency by tailoring the precision of computation adaptively to temporal changes in algorithmic noise tolerance. DPS can decrease the arithmetic precision of noise-tolerant phases to result in power savings at the same operating speed (or faster execution within the same power budget), while keeping the overall loss in accuracy due to precision reduction bounded.

==> appEvalFig.tex <==
\begin{figure*}[htp]
%\label{fig:bit_maps}
  \begin{center}
	\subfloat[BS]{
	  \includegraphics[width=0.33\columnwidth]{bs_map}
    }
	\subfloat[FA]{
	  \includegraphics[width=0.33\columnwidth]{fa_map}
    }
	\subfloat[HS]{
	  \includegraphics[width=0.33\columnwidth]{hs_map}
    }\\
	\subfloat[PF]{
	  \includegraphics[width=0.33\columnwidth]{pf_map}
    }
	\subfloat[PR]{
	  \includegraphics[width=0.33\columnwidth]{pr_map}
    }
	\caption{Profiling outcome for temporal noise tolerance.
	  \label{fig:profile}}
  \end{center}
\vspace{-0.1cm}
\end{figure*}




==> intro.tex <==
Practical stagnation in voltage scaling renders an increasing chip power density
(power per area) over technology generations.  At the same time, cooling and
power delivery limitations prevent a proportional expansion of the chip power
budget.  The only way to sustain performance improvement in this environment is
enhancing power efficiency, i.e., performance gain per unit power
consumed~\cite{Horow}.  {\em Approximate computing} is a promising paradigm
which can enhance power efficiency by trading computation accuracy for
performance or power, depending on the tolerance of algorithms to noise (i.e.,
accuracy loss) in computation.  The intrinsic noise tolerance of the emerging
R(ecognition), M(ining), and S(ynthesis) applications~\cite{rms} -- which
process massive but noisy input data by probabilistic algorithms (often
featuring iterative refinement) -- makes them particularly suitable to
approximate computing. 

Approximate computing by precision reduction represents a heavily explored area
of research~\cite{yeh2007,discApprox,enerJ}.  In this paper, we explore
approximation by {\em adaptive} precision reduction, a relatively less explored
area.  Specifically, based on the observation that applications exhibit varying
degrees of sensitivity to noise during computation, we explore {\em how
tailoring the precision of computation adaptively to temporal changes in
algorithmic noise tolerance can maximize power efficiency}. 

Due to its analogy to Dynamic Voltage and Frequency Scaling (DVFS), we refer to
this paradigm as {\em Dynamic Precision Scaling} (DPS).
Recall that DVFS can maximize power efficiency by tracking temporal changes in the
performance demand of the workload (which in turn evolves as a function of
temporal changes in computation and memory access characteristics) and by
changing the operating point (i.e., the operating voltage and frequency)
accordingly. 
Similar to DVFS, DPS tracks temporal changes in workload characteristics.
However, in maximizing power efficiency, contrary to DVFS, DPS exploits temporal
changes in noise tolerance, and adaptively decreases the arithmetic precision of
noise-tolerant phases to obtain power savings at the same operating speed (or
faster execution within the same power budget) while keeping the overall loss in
accuracy due to precision reduction bounded.  \redHL{Conceptually,} for less noise-tolerant phases,
DPS can adjust the arithmetic precision on the fly to prevent excessive loss in
computation accuracy.

\redHL{In this paper, we conduct a limit study 
in order to quantify the power efficiency potential of DPS. To this end, we
devise a proof-of-concept implementation of the DPS concept.
Specifically,} we first develop
a workload analyzer which can identify application phases of varying noise
tolerance. Then, using the outcome of this workload analyzer, we design two
heuristic DPS policies.  In the following, 
Section~\ref{sec:dps} introduces DPS basics and the two \redHL{proof-of-concept} policies;
Sections~\ref{sec:setup} and~\ref{sec:eval} provide the evaluation;
Section~\ref{sec:rel} covers related work; 
and Section~\ref{sec:conc} summarizes our findings.




==> rel.tex <==
Static precision reduction for floating point arithmetic has been heavily
studied (e.g.,~\cite{rutenbar}).  Adaptive precision reduction, on the other
hand, has been explored in the context of physics simulation to minimize the
area cost of floating point units (FPUs)~\cite{yeh2007} and for digital signal
processing~\cite{dspDPS}.  In contrast, our focus is to show the opportunity in
general purpose computing.  Our study evaluates DPS for floating point
approximation, however, DPS can be applied to the integer data path, as well.
At the same time, our goal is boosting the power efficiency considering a
broader emerging class of RMS applications~\cite{rms}.  Automated program
analysis tools to help developers tune floating point
precision~\cite{preci,linderman} fit well into the {\em offline profiling} stage
of DPS, but the existing body of work in this domain usually does not explore
adaptive precision tuning at runtime.

One end of the spectrum for detection of approximation in software is
EnerJ~\cite{enerJ}.  In this work, the authors do not automate the process and
require programmers to define approximate data types.  On the other hand,
Chisel~\cite{chisel} provides a semi-automated approach which tries to maximize
both accuracy and energy efficiency at the same time.  However, Chisel still
requires the programmer to specify approximate program segments and probability
that the specified function should execute correctly.  In our approach, we are
trying to detect possible noise tolerant phases automatically.  Proposed
methodology in this work can be used to detect and reduce the time spend to tune
the approximate code segments for ~\cite{enerJ} and ~\cite{chisel}.

As oppose to semi or non-automated mechanisms, SAGE~\cite{sage} proposes an
automated approach by using online monitoring mechanism designed for GPU
kernels.  Closest to our work, Approxilyzer~\cite{approxilyzer} tries to find
noise tolerant instructions in an application and classifies them as Masked,
SDC-Good/Maybe/Bad, and detectable errors.  This approach is automated; however,
it is only limited to single bit errors.  In this work, we expand the code
region and work on the function granularity to enable more energy reduction. 

In addition to the holistic approximate computing approaches, configurable
approximate floating point arithmetic units attracted significant attention
~\cite{fpmul1}, ~\cite{fpmul2}. 


